Vaporetto: Efficient Japanese Tokenization Based on Improved Pointwise Linear Classification

This paper proposes an approach to improve the runtime efficiency of Japanese tokenization based on the pointwise linear classification (PLC) framework, which formulates the whole tokenization process as a sequence of linear classification problems. Our approach optimizes tokenization by leveraging the characteristics of the PLC framework and the task definition. Our approach involves (1) composing multiple classifications into array-based operations, (2) efficient feature lookup with memory-optimized automata, and (3) three orthogonal pre-processing methods for reducing actual score calculation. Thus, our approach makes the tokenization speed 5.7 times faster than the current approach based on the same model without decreasing tokenization accuracy. Our implementation is available at https://github.com/daac-tools/vaporetto under the MIT or Apache-2.0 license.

==> author-response.tex <==
\section{Author Response}

Several reviewers asked about applicability to other languages. We will address this point in the Limitations section.
Also, we will cite suggested previous works in the paper.

\paragraph{Q:}
There is no empirical evidence to validate tokenization accuracy in the experiments, where only the processing speed of various methods is carefully evaluated.

\paragraph{A:}
In order to design the method described in Section 3.3, we slightly changed dictionary features from KyTea. However, this change has only a trivial impact on the tokenization accuracy. We will explain the change in the Appendix.

\paragraph{Q:}
Does the speed improvement has anything to do with its Rust implementation?

\paragraph{A:}
Since both C++ and Rust are system programming languages, both compilers generate similar assemblies if the standard library is not used.
We did not use the standard library in the main part of our methods, so we do not think that a significant change in speed occurs whether implemented in C++ or Rust.

\paragraph{Q:}
It is unclear that the current system achieves speedup without sacrificing accuracy compared with lattice-based systems.

\paragraph{A:}
The purpose of this study is not to compare the accuracy of PLC and lattice methods.
KyTea's paper shows that the PLC method improves the efficiency of domain adaptation by the partial annotation framework. Both methods have unique characteristics and are used in different situations. The accuracy comparison in Section 1 and the speed comparison in Section 4.2 are for reference only and are not intended to discuss the advantages of the PLC method.
We will add further explanations of the differences between PLC and lattice methods.
The speed comparison of KyTea and MeCab in Section 1 is based on our experimental results (Section 4.3, Table 1). We refer to Table 1 in Section 1.

\paragraph{Q:}
There is no clear description of the algorithm used as the foundation of the reported work.

\paragraph{A:}
We will add the following description at the last of Section 2 to clarify our work: KyTea is a straightforward implementation of Algorithm 1, and there is room for several improvements in time efficiency.
One is the pattern match function Match$(\bm{a})$ (line 2).
Another is the process of calculating scores (line 8).

\paragraph{Q:}
The concept of ``failure edges'' is not explained sufficiently clearly. A more detailed description of the AC (Aho-Corasick) algorithm would be of benefit.

\paragraph{A:}
It would be difficult to give a detailed description of the AC algorithm due to the space limitation. So, we will modify ``failure edges'' into ``failure transitions'' used in the original paper (Aho and Corasick, 1975) and add a citation to the paper.

\paragraph{Q:}
The contribution depends on data that are simply not available outside the author's institution or consortium and/or not enough details are provided.

\paragraph{A:}
We used BCCWJ and UniDic for experiments. BCCWJ is not open source and requires a usage fee. However, both are the most widely used datasets in Japanese natural language processing, and we do not think our work is unreproducible. In the field of word segmentation, UniDic is used by Neubig et al. (2011) and Takaoka et al. (2018); and is also mentioned by Tolmachev et al. (2019). BCCWJ is used by Neubig et al. (2011) and mentioned by Takaoka et al. (2018). Also, BCCWJ is used in the word sense disambiguation task in SemEval-2010 (Okumura et al., 2010).
